Two-Body Motion in Central Conservative Force Fields

The two-body motion for the gravitational and linear elastic central conservative force field is discussed by comparing the differential equations of motions. The inverse and direct square displacement dependency of the two force types is shown as emerging in the trajectories. The closed (for the gravitational field) and open (for the particular dumbbell elastic system considered) character of the trajectory is discussed.

==> rrp_mathdefs.tex <==
%\newcommand{\opL}{\mathfrak{L}}
%\newcommand{\opN}{\mathfrak{N}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

\newcommand{\ddiv}{\ensuremath{\mathop{\operator@font div}\nolimits}}
\newcommand{\grad}{\ensuremath{\mathop{\operator@font grad}\nolimits}}
\newcommand{\artanh}{\ensuremath{\mathop{\operator@font artanh}\nolimits}}
\newcommand{\sech}{\ensuremath{\mathop{\operator@font sech}\nolimits}}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}

\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

